Dense Multitask Learning to Reconfigure Comics

In this paper, we develop a MultiTask Learning (MTL) model to achieve dense predictions for comics panels to, in turn, facilitate the transfer of comics from one publication channel to another by assisting authors in the task of reconfiguring their narratives. Our MTL method can successfully identify the semantic units as well as the embedded notion of 3D in comic panels. This is a significantly challenging problem because comics comprise disparate artistic styles, illustrations, layouts, and object scales that depend on the authors creative process. Typically, dense image-based prediction techniques require a large corpus of data. Finding an automated solution for dense prediction in the comics domain, therefore, becomes more difficult with the lack of ground-truth dense annotations for the comics images. To address these challenges, we develop the following solutions: 1) we leverage a commonly-used strategy known as unsupervised image-to-image translation, which allows us to utilize a large corpus of real-world annotations; 2) we utilize the results of the translations to develop our multitasking approach that is based on a vision transformer backbone and a domain transferable attention module; 3) we study the feasibility of integrating our MTL dense-prediction method with an existing retargeting method, thereby reconfiguring comics.

==> images/teaser.tex <==
\begin{center}
\centering
  \includegraphics %[width=0.47\textwidth]{mainpaper/images/teaser-MulT-overview.png}
  \includegraphics[height= 5.0cm, width= 9.0cm]{mainpaper/images/teaser-comparison.png}
  \captionof{figure}{\textbf{Overview of MulT.} (Left) In our MulT framework, we jointly train multiple vision tasks, using a single encoder and a consistent decoder architecture with a task specific decoder head. The shared attention in our framework, further facilitates the joint learning between the multiple tasks. (Right)~ Our MulT model produces better results than both the single dedicated task models (Single task transformer) and the Multitask CNN baseline~\cite{standley2019}. Best seen on screen and zoomed in.}%
\label{fig:teaser}
\end{center}
